Exploring Graph Neural Networks for Indian Legal Judgment Prediction

The burdensome impact of a skewed judges-to-cases ratio on the judicial system manifests in an overwhelming backlog of pending cases alongside an ongoing influx of new ones. To tackle this issue and expedite the judicial process, the proposition of an automated system capable of suggesting case outcomes based on factual evidence and precedent from past cases gains significance. This research paper centres on developing a graph neural network-based model to address the Legal Judgment Prediction (LJP) problem, recognizing the intrinsic graph structure of judicial cases and making it a binary node classification problem. We explored various embeddings as model features, while nodes such as time nodes and judicial acts were added and pruned to evaluate the model's performance. The study is done while considering the ethical dimension of fairness in these predictions, considering gender and name biases. A link prediction task is also conducted to assess the model's proficiency in anticipating connections between two specified nodes. By harnessing the capabilities of graph neural networks and incorporating fairness analyses, this research aims to contribute insights towards streamlining the adjudication process, enhancing judicial efficiency, and fostering a more equitable legal landscape, ultimately alleviating the strain imposed by mounting case backlogs. Our best-performing model with XLNet pre-trained embeddings as its features gives the macro F1 score of 75% for the LJP task. For link prediction, the same set of features is the best performing giving ROC of more than 80%

==> link_prediction/tex/hierar.tex <==
% This file was created with tikzplotlib v0.9.12.
\begin{tikzpicture}

\begin{groupplot}[group style={group size=2 by 2}]
\nextgroupplot[
axis background/.style={fill=white!89.8039215686275!black},
axis line style={white},
tick align=outside,
tick pos=left,
title={Remove Acts
},
x grid style={white},
xmajorgrids,
xmin=-0.55, xmax=11.55,
xtick style={color=white!33.3333333333333!black},
xtick={0,1,2,3,4,5,6,7,8,9,10,11},
xtick={0,1,2,3,4,5,6,7,8,9,10,11},
xtick={0,1,2,3,4,5,6,7,8,9,10,11},
xtick={0,1,2,3,4,5,6,7,8,9,10,11},
xtick={0,1,2,3,4,5,6,7,8,9,10,11},
xtick={0,1,2,3,4,5,6,7,8,9,10,11},
xtick={0,1,2,3,4,5,6,7,8,9,10,11},
xticklabels={1956,1961,1966,1971,1976,1981,1986,1991,1996,2001,2006,2011},
xticklabels={1956,1961,1966,1971,1976,1981,1986,1991,1996,2001,2006,2011},
xticklabels={1956,1961,1966,1971,1976,1981,1986,1991,1996,2001,2006,2011},
xticklabels={1956,1961,1966,1971,1976,1981,1986,1991,1996,2001,2006,2011},
xticklabels={1956,1961,1966,1971,1976,1981,1986,1991,1996,2001,2006,2011},
xticklabels={1956,1961,1966,1971,1976,1981,1986,1991,1996,2001,2006,2011},
xticklabels={1956,1961,1966,1971,1976,1981,1986,1991,1996,2001,2006,2011},
y grid style={white},
ymajorgrids,
ymin=-0.04904, ymax=1.02984,
ytick style={color=white!33.3333333333333!black},
ytick={-0.2,0,0.2,0.4,0.6,0.8,1,1.2},
yticklabels={−0.2,0.0,0.2,0.4,0.6,0.8,1.0,1.2}
]
\addplot [red, dotted]
table {%
0 0.8479
1 0.7956
2 0.7892
3 0.7806
4 0.785
5 0.7915
6 0.7917
7 0.791
8 0.8009
9 0.7954
10 0.7967
11 0
};
\addplot [red]
table {%
0 0.7788
1 0.7683
2 0.756
3 0.7433
4 0.7491
5 0.7632
6 0.7462
7 0.7657
8 0.8989
9 0.8905
10 0
11 0
};
\addplot [very thick, blue, dotted]
table {%
0 0.9372
1 0.9194
2 0.9175
3 0.9055
4 0.9056
5 0.8993
6 0.9062
7 0.9043
8 0.9071
9 0.9153
10 0.9229
11 0
};
\addplot [very thick, blue]
table {%
0 0.8916
1 0.9038
2 0.8999
3 0.9056
4 0.9123
5 0.9196
6 0.9295
7 0.9543
8 0.9727
9 0.9808
10 0
11 0
};
\addplot [thick, black, dotted]
table {%
0 0.8046
1 0.8223
2 0.8223
3 0.8222
4 0.8281
5 0.8207
6 0.8087
7 0.8156
8 0.8266
9 0.8337
10 0.8307
11 0
};
\addplot [thick, black]
table {%
0 0.7961
1 0.793
2 0.8115
3 0.812
4 0.8294
5 0.8321
6 0.8317
7 0.8846
8 0.8921
9 0.8624
10 0
11 0
};

\nextgroupplot[
axis background/.style={fill=white!89.8039215686275!black},
axis line style={white},
tick align=outside,
tick pos=left,
title={Keep Acts
},
x grid style={white},
xmajorgrids,
xmin=-0.55, xmax=11.55,
xtick style={color=white!33.3333333333333!black},
xtick={0,1,2,3,4,5,6,7,8,9,10,11},
xtick={0,1,2,3,4,5,6,7,8,9,10,11},
xtick={0,1,2,3,4,5,6,7,8,9,10,11},
xtick={0,1,2,3,4,5,6,7,8,9,10,11},
xtick={0,1,2,3,4,5,6,7,8,9,10,11},
xtick={0,1,2,3,4,5,6,7,8,9,10,11},
xtick={0,1,2,3,4,5,6,7,8,9,10,11},
xticklabel style={rotate=90.0},
xticklabels={1956,1961,1966,1971,1976,1981,1986,1991,1996,2001,2006,2011},
xticklabels={1956,1961,1966,1971,1976,1981,1986,1991,1996,2001,2006,2011},
xticklabels={1956,1961,1966,1971,1976,1981,1986,1991,1996,2001,2006,2011},
xticklabels={1956,1961,1966,1971,1976,1981,1986,1991,1996,2001,2006,2011},
xticklabels={1956,1961,1966,1971,1976,1981,1986,1991,1996,2001,2006,2011},
xticklabels={1956,1961,1966,1971,1976,1981,1986,1991,1996,2001,2006,2011},
xticklabels={1956,1961,1966,1971,1976,1981,1986,1991,1996,2001,2006,2011},
y grid style={white},
ylabel={Yes Time

ROC\_AUC},
ymajorgrids,
ymin=-0.047345, ymax=1,
ytick style={color=white!33.3333333333333!black},
ytick={0,0.05,0.1,0.15,0.2,0.25,0.3,0.35,0.4,0.45,0.5,0.55,0.6,0.65,0.7,0.75,0.8,0.85,0.9,0.95,1},
yticklabels={0.0,0.05,0.1,0.15,0.2,0.25,0.3,0.35,0.4,0.45,0.5,0.55,0.6,0.65,0.7,0.75,0.8,0.85,0.9,0.95,1.0}
]
\addplot [red, dotted]
table {%
0 0.7759
1 0.7643
2 0.7595
3 0.7597
4 0.7632
5 0.7604
6 0.7595
7 0.7658
8 0.7578
9 0.7611
10 0.7665
11 0
};
\addplot [red]
table {%
0 0.7366
1 0.696
2 0.705
3 0.7032
4 0.7352
5 0.7377
6 0.7309
7 0.7602
8 0.7999
9 0.7825
10 0
11 0
};
\addplot [very thick, blue, dotted]
table {%
0 0.9341
1 0.9244
2 0.9278
3 0.9224
4 0.9201
5 0.9198
6 0.9149
7 0.9028
8 0.9062
9 0.8966
10 0.8973
11 0
};
\addplot [very thick, blue]
table {%
0 0.9085
1 0.9092
2 0.917
3 0.9232
4 0.9311
5 0.9301
6 0.9221
7 0.932
8 0.9436
9 0.9469
10 0
11 0
};
\addplot [thick, black, dotted]
table {%
0 0.8513
1 0.8433
2 0.8321
3 0.8315
4 0.833
5 0.8262
6 0.8451
7 0.8265
8 0.8137
9 0.8207
10 0.8109
11 0
};
\addplot [thick, black]
table {%
0 0.8294
1 0.8323
2 0.8185
3 0.8362
4 0.8439
5 0.8511
6 0.8402
7 0.8639
8 0.8507
9 0.8512
10 0
11 0
};

\nextgroupplot[
axis background/.style={fill=white!89.8039215686275!black},
axis line style={white},
tick align=outside,
tick pos=left,
x grid style={white},
xmajorgrids,
xmin=-0.55, xmax=11.55,
xtick style={color=white!33.3333333333333!black},
xtick={0,1,2,3,4,5,6,7,8,9,10,11},
xtick={0,1,2,3,4,5,6,7,8,9,10,11},
xtick={0,1,2,3,4,5,6,7,8,9,10,11},
xtick={0,1,2,3,4,5,6,7,8,9,10,11},
xtick={0,1,2,3,4,5,6,7,8,9,10,11},
xtick={0,1,2,3,4,5,6,7,8,9,10,11},
xtick={0,1,2,3,4,5,6,7,8,9,10,11},
xticklabel style={rotate=90.0},
xticklabels={1956,1961,1966,1971,1976,1981,1986,1991,1996,2001,2006,2011},
xticklabels={1956,1961,1966,1971,1976,1981,1986,1991,1996,2001,2006,2011},
xticklabels={1956,1961,1966,1971,1976,1981,1986,1991,1996,2001,2006,2011},
xticklabels={1956,1961,1966,1971,1976,1981,1986,1991,1996,2001,2006,2011},
xticklabels={1956,1961,1966,1971,1976,1981,1986,1991,1996,2001,2006,2011},
xticklabels={1956,1961,1966,1971,1976,1981,1986,1991,1996,2001,2006,2011},
xticklabels={1956,1961,1966,1971,1976,1981,1986,1991,1996,2001,2006,2011},
y grid style={white},
ymajorgrids,
ymin=-0.04865, ymax=1.02165,
ytick style={color=white!33.3333333333333!black},
ytick={-0.2,0,0.2,0.4,0.6,0.8,1,1.2},
yticklabels={−0.2,0.0,0.2,0.4,0.6,0.8,1.0,1.2}
]
\addplot [red, dotted]
table {%
0 0.8729
1 0.846
2 0.8309
3 0.8193
4 0.8281
5 0.8351
6 0.8461
7 0.8471
8 0.8525
9 0.8522
10 0.8509
11 0
};
\addplot [red]
table {%
0 0.838
1 0.8167
2 0.7987
3 0.798
4 0.802
5 0.8293
6 0.8647
7 0.9084
8 0.9632
9 0.973
10 0
11 0
};
\addplot [very thick, blue, dotted]
table {%
0 0.9355
1 0.9255
2 0.9235
3 0.9149
4 0.9143
5 0.9136
6 0.9107
7 0.9178
8 0.914
9 0.9181
10 0.9216
11 0
};
\addplot [very thick, blue]
table {%
0 0.9255
1 0.917
2 0.9198
3 0.9206
4 0.919
5 0.9237
6 0.9252
7 0.9278
8 0.9565
9 0.9435
10 0
11 0
};
\addplot [thick, black, dotted]
table {%
0 0.8081
1 0.8184
2 0.8219
3 0.83
4 0.829
5 0.8244
6 0.8233
7 0.8298
8 0.8196
9 0.8185
10 0.8146
11 0
};
\addplot [thick, black]
table {%
0 0.8125
1 0.8158
2 0.8196
3 0.8232
4 0.8204
5 0.817
6 0.808
7 0.8252
8 0.8588
9 0.8609
10 0
11 0
};
\end{groupplot}

\begin{groupplot}[group style={group size=2 by 2}]
\nextgroupplot[
axis background/.style={fill=white!89.8039215686275!black},
axis line style={white},
tick align=outside,
tick pos=left,
x grid style={white},
xmajorgrids,
xmin=-0.55, xmax=11.55,
xtick style={color=white!33.3333333333333!black},
xtick={0,1,2,3,4,5,6,7,8,9,10,11},
xtick={0,1,2,3,4,5,6,7,8,9,10,11},
xtick={0,1,2,3,4,5,6,7,8,9,10,11},
xtick={0,1,2,3,4,5,6,7,8,9,10,11},
xtick={0,1,2,3,4,5,6,7,8,9,10,11},
xtick={0,1,2,3,4,5,6,7,8,9,10,11},
xtick={0,1,2,3,4,5,6,7,8,9,10,11},
xticklabel style={rotate=90.0},
xticklabels={1956,1961,1966,1971,1976,1981,1986,1991,1996,2001,2006,2011},
xticklabels={1956,1961,1966,1971,1976,1981,1986,1991,1996,2001,2006,2011},
xticklabels={1956,1961,1966,1971,1976,1981,1986,1991,1996,2001,2006,2011},
xticklabels={1956,1961,1966,1971,1976,1981,1986,1991,1996,2001,2006,2011},
xticklabels={1956,1961,1966,1971,1976,1981,1986,1991,1996,2001,2006,2011},
xticklabels={1956,1961,1966,1971,1976,1981,1986,1991,1996,2001,2006,2011},
xticklabels={1956,1961,1966,1971,1976,1981,1986,1991,1996,2001,2006,2011},
y grid style={white},
ylabel={No Time

ROC\_AUC},
ymajorgrids,
ymin=-0.04745, ymax=1,
ytick style={color=white!33.3333333333333!black},
ytick={0,0.05,0.1,0.15,0.2,0.25,0.3,0.35,0.4,0.45,0.5,0.55,0.6,0.65,0.7,0.75,0.8,0.85,0.9,0.95,1},
yticklabels={0.0,0.05,0.1,0.15,0.2,0.25,0.3,0.35,0.4,0.45,0.5,0.55,0.6,0.65,0.7,0.75,0.8,0.85,0.9,0.95,1.0}
]
\addplot [red, dotted]
table {%
0 0.781
1 0.7891
2 0.7764
3 0.7732
4 0.7749
5 0.7744
6 0.7805
7 0.7805
8 0.7784
9 0.7827
10 0.7821
11 0
};
\addplot [red]
table {%
0 0.753
1 0.7485
2 0.7637
3 0.7531
4 0.7601
5 0.7919
6 0.7863
7 0.7514
8 0.8088
9 0.8018
10 0
11 0
};
\addplot [very thick, blue, dotted]
table {%
0 0.9343
1 0.9288
2 0.9255
3 0.9282
4 0.9168
5 0.9119
6 0.9113
7 0.9103
8 0.89
9 0.8835
10 0.8798
11 0
};
\addplot [very thick, blue]
table {%
0 0.8952
1 0.9084
2 0.9129
3 0.9112
4 0.9249
5 0.9302
6 0.9348
7 0.9434
8 0.949
9 0.938
10 0
11 0
};
\addplot [thick, black, dotted]
table {%
0 0.8544
1 0.853
2 0.8466
3 0.8472
4 0.8444
5 0.8417
6 0.844
7 0.8543
8 0.8226
9 0.8252
10 0.821
11 0
};
\addplot [thick, black]
table {%
0 0.8414
1 0.8422
2 0.8436
3 0.8511
4 0.8587
5 0.8635
6 0.8614
7 0.8806
8 0.8656
9 0.8504
10 0
11 0
};
\draw ({$(current bounding box.south west)!0.5!(current bounding box.south east)$}|-{$(current bounding box.south west)!0.98!(current bounding box.north west)$}) node[
  scale=0.6,
  anchor=north,
  text=black,
  rotate=0.0
]{hierar};
\end{groupplot}

\end{tikzpicture}


==> link_prediction/tex/pretrained.tex <==
% This file was created with tikzplotlib v0.9.12.
\begin{tikzpicture}

\begin{groupplot}[group style={group size=2 by 2}]
\nextgroupplot[
axis background/.style={fill=white!89.8039215686275!black},
axis line style={white},
tick align=outside,
tick pos=left,
title={Remove Acts
},
x grid style={white},
xmajorgrids,
xmin=-0.55, xmax=11.55,
xtick style={color=white!33.3333333333333!black},
xtick={0,1,2,3,4,5,6,7,8,9,10,11},
xtick={0,1,2,3,4,5,6,7,8,9,10,11},
xtick={0,1,2,3,4,5,6,7,8,9,10,11},
xtick={0,1,2,3,4,5,6,7,8,9,10,11},
xtick={0,1,2,3,4,5,6,7,8,9,10,11},
xtick={0,1,2,3,4,5,6,7,8,9,10,11},
xtick={0,1,2,3,4,5,6,7,8,9,10,11},
xticklabels={1956,1961,1966,1971,1976,1981,1986,1991,1996,2001,2006,2011},
xticklabels={1956,1961,1966,1971,1976,1981,1986,1991,1996,2001,2006,2011},
xticklabels={1956,1961,1966,1971,1976,1981,1986,1991,1996,2001,2006,2011},
xticklabels={1956,1961,1966,1971,1976,1981,1986,1991,1996,2001,2006,2011},
xticklabels={1956,1961,1966,1971,1976,1981,1986,1991,1996,2001,2006,2011},
xticklabels={1956,1961,1966,1971,1976,1981,1986,1991,1996,2001,2006,2011},
xticklabels={1956,1961,1966,1971,1976,1981,1986,1991,1996,2001,2006,2011},
y grid style={white},
ymajorgrids,
ymin=-0.048565, ymax=1.019865,
ytick style={color=white!33.3333333333333!black},
ytick={-0.2,0,0.2,0.4,0.6,0.8,1,1.2},
yticklabels={−0.2,0.0,0.2,0.4,0.6,0.8,1.0,1.2}
]
\addplot [red, dotted]
table {%
0 0.8602
1 0.8236
2 0.8047
3 0.7938
4 0.8038
5 0.8076
6 0.8095
7 0.7947
8 0.7942
9 0.7941
10 0.7929
11 0.7954
};
\addplot [red]
table {%
0 0.7839
1 0.7882
2 0.7734
3 0.7877
4 0.7971
5 0.7999
6 0.8087
7 0.8302
8 0.8918
9 0.9341
10 0.9202
11 0
};
\addplot [very thick, blue, dotted]
table {%
0 0.9363
1 0.9338
2 0.9221
3 0.9235
4 0.9178
5 0.9167
6 0.9197
7 0.9216
8 0.9152
9 0.9171
10 0.921
11 0.9261
};
\addplot [very thick, blue]
table {%
0 0.9249
1 0.9244
2 0.9247
3 0.9202
4 0.9315
5 0.9272
6 0.9374
7 0.9447
8 0.9561
9 0.9477
10 0.9713
11 0
};
\addplot [thick, black, dotted]
table {%
0 0.7897
1 0.8054
2 0.8206
3 0.8154
4 0.8226
5 0.8283
6 0.8331
7 0.8333
8 0.8205
9 0.826
10 0.8291
11 0.8343
};
\addplot [thick, black]
table {%
0 0.8164
1 0.8193
2 0.8225
3 0.8253
4 0.8241
5 0.8187
6 0.8177
7 0.8084
8 0.7613
9 0.8083
10 0.8407
11 0
};

\nextgroupplot[
axis background/.style={fill=white!89.8039215686275!black},
axis line style={white},
tick align=outside,
tick pos=left,
title={Keep Acts
},
x grid style={white},
xmajorgrids,
xmin=-0.55, xmax=11.55,
xtick style={color=white!33.3333333333333!black},
xtick={0,1,2,3,4,5,6,7,8,9,10,11},
xtick={0,1,2,3,4,5,6,7,8,9,10,11},
xtick={0,1,2,3,4,5,6,7,8,9,10,11},
xtick={0,1,2,3,4,5,6,7,8,9,10,11},
xtick={0,1,2,3,4,5,6,7,8,9,10,11},
xtick={0,1,2,3,4,5,6,7,8,9,10,11},
xtick={0,1,2,3,4,5,6,7,8,9,10,11},
xticklabel style={rotate=90.0},
xticklabels={1956,1961,1966,1971,1976,1981,1986,1991,1996,2001,2006,2011},
xticklabels={1956,1961,1966,1971,1976,1981,1986,1991,1996,2001,2006,2011},
xticklabels={1956,1961,1966,1971,1976,1981,1986,1991,1996,2001,2006,2011},
xticklabels={1956,1961,1966,1971,1976,1981,1986,1991,1996,2001,2006,2011},
xticklabels={1956,1961,1966,1971,1976,1981,1986,1991,1996,2001,2006,2011},
xticklabels={1956,1961,1966,1971,1976,1981,1986,1991,1996,2001,2006,2011},
xticklabels={1956,1961,1966,1971,1976,1981,1986,1991,1996,2001,2006,2011},
y grid style={white},
ylabel={Yes Time

ROC\_AUC},
ymajorgrids,
ymin=-0.04771, ymax=1.00191,
ytick style={color=white!33.3333333333333!black},
ytick={0,0.05,0.1,0.15,0.2,0.25,0.3,0.35,0.4,0.45,0.5,0.55,0.6,0.65,0.7,0.75,0.8,0.85,0.9,0.95,1},
yticklabels={0.0,0.05,0.1,0.15,0.2,0.25,0.3,0.35,0.4,0.45,0.5,0.55,0.6,0.65,0.7,0.75,0.8,0.85,0.9,0.95,1.0}
]
\addplot [red, dotted]
table {%
0 0.7795
1 0.7836
2 0.775
3 0.7767
4 0.7758
5 0.7761
6 0.7717
7 0.7721
8 0.7531
9 0.7534
10 0.7524
11 0.7498
};
\addplot [red]
table {%
0 0.7452
1 0.7353
2 0.7326
3 0.742
4 0.755
5 0.7776
6 0.7783
7 0.7707
8 0.7954
9 0.7981
10 0.8889
11 0
};
\addplot [very thick, blue, dotted]
table {%
0 0.9376
1 0.9329
2 0.9294
3 0.9261
4 0.931
5 0.9221
6 0.9266
7 0.9317
8 0.9045
9 0.9112
10 0.9028
11 0.911
};
\addplot [very thick, blue]
table {%
0 0.9263
1 0.9349
2 0.934
3 0.9331
4 0.9401
5 0.9416
6 0.9468
7 0.9517
8 0.942
9 0.946
10 0.9542
11 0
};
\addplot [thick, black, dotted]
table {%
0 0.8454
1 0.854
2 0.8438
3 0.8475
4 0.8463
5 0.8529
6 0.8473
7 0.8534
8 0.8245
9 0.813
10 0.8223
11 0.8045
};
\addplot [thick, black]
table {%
0 0.8425
1 0.8546
2 0.8562
3 0.8602
4 0.8605
5 0.8646
6 0.87
7 0.8824
8 0.8549
9 0.8641
10 0.7694
11 0
};

\nextgroupplot[
axis background/.style={fill=white!89.8039215686275!black},
axis line style={white},
tick align=outside,
tick pos=left,
x grid style={white},
xmajorgrids,
xmin=-0.55, xmax=11.55,
xtick style={color=white!33.3333333333333!black},
xtick={0,1,2,3,4,5,6,7,8,9,10,11},
xtick={0,1,2,3,4,5,6,7,8,9,10,11},
xtick={0,1,2,3,4,5,6,7,8,9,10,11},
xtick={0,1,2,3,4,5,6,7,8,9,10,11},
xtick={0,1,2,3,4,5,6,7,8,9,10,11},
xtick={0,1,2,3,4,5,6,7,8,9,10,11},
xtick={0,1,2,3,4,5,6,7,8,9,10,11},
xticklabel style={rotate=90.0},
xticklabels={1956,1961,1966,1971,1976,1981,1986,1991,1996,2001,2006,2011},
xticklabels={1956,1961,1966,1971,1976,1981,1986,1991,1996,2001,2006,2011},
xticklabels={1956,1961,1966,1971,1976,1981,1986,1991,1996,2001,2006,2011},
xticklabels={1956,1961,1966,1971,1976,1981,1986,1991,1996,2001,2006,2011},
xticklabels={1956,1961,1966,1971,1976,1981,1986,1991,1996,2001,2006,2011},
xticklabels={1956,1961,1966,1971,1976,1981,1986,1991,1996,2001,2006,2011},
xticklabels={1956,1961,1966,1971,1976,1981,1986,1991,1996,2001,2006,2011},
y grid style={white},
ymajorgrids,
ymin=-0.04791, ymax=1.00611,
ytick style={color=white!33.3333333333333!black},
ytick={-0.2,0,0.2,0.4,0.6,0.8,1,1.2},
yticklabels={−0.2,0.0,0.2,0.4,0.6,0.8,1.0,1.2}
]
\addplot [red, dotted]
table {%
0 0.8785
1 0.8479
2 0.8375
3 0.836
4 0.8475
5 0.8505
6 0.8515
7 0.8493
8 0.8503
9 0.8509
10 0.8503
11 0.8498
};
\addplot [red]
table {%
0 0.841
1 0.8337
2 0.8293
3 0.8238
4 0.8359
5 0.8437
6 0.8602
7 0.8751
8 0.9366
9 0.9495
10 0.9204
11 0
};
\addplot [very thick, blue, dotted]
table {%
0 0.9364
1 0.9347
2 0.9268
3 0.9302
4 0.9288
5 0.9278
6 0.9261
7 0.9294
8 0.9213
9 0.9182
10 0.9227
11 0.9177
};
\addplot [very thick, blue]
table {%
0 0.9299
1 0.9298
2 0.9298
3 0.9347
4 0.9392
5 0.9392
6 0.9358
7 0.9456
8 0.9333
9 0.9397
10 0.9582
11 0
};
\addplot [thick, black, dotted]
table {%
0 0.8072
1 0.8239
2 0.8297
3 0.8363
4 0.8395
5 0.8378
6 0.8368
7 0.8369
8 0.8293
9 0.8289
10 0.823
11 0.823
};
\addplot [thick, black]
table {%
0 0.8281
1 0.8335
2 0.8307
3 0.8382
4 0.8331
5 0.8311
6 0.8156
7 0.8078
8 0.7935
9 0.7814
10 0.834
11 0
};
\end{groupplot}

\begin{groupplot}[group style={group size=2 by 2}]
\nextgroupplot[
axis background/.style={fill=white!89.8039215686275!black},
axis line style={white},
tick align=outside,
tick pos=left,
x grid style={white},
xmajorgrids,
xmin=-0.55, xmax=11.55,
xtick style={color=white!33.3333333333333!black},
xtick={0,1,2,3,4,5,6,7,8,9,10,11},
xtick={0,1,2,3,4,5,6,7,8,9,10,11},
xtick={0,1,2,3,4,5,6,7,8,9,10,11},
xtick={0,1,2,3,4,5,6,7,8,9,10,11},
xtick={0,1,2,3,4,5,6,7,8,9,10,11},
xtick={0,1,2,3,4,5,6,7,8,9,10,11},
xtick={0,1,2,3,4,5,6,7,8,9,10,11},
xticklabel style={rotate=90.0},
xticklabels={1956,1961,1966,1971,1976,1981,1986,1991,1996,2001,2006,2011},
xticklabels={1956,1961,1966,1971,1976,1981,1986,1991,1996,2001,2006,2011},
xticklabels={1956,1961,1966,1971,1976,1981,1986,1991,1996,2001,2006,2011},
xticklabels={1956,1961,1966,1971,1976,1981,1986,1991,1996,2001,2006,2011},
xticklabels={1956,1961,1966,1971,1976,1981,1986,1991,1996,2001,2006,2011},
xticklabels={1956,1961,1966,1971,1976,1981,1986,1991,1996,2001,2006,2011},
xticklabels={1956,1961,1966,1971,1976,1981,1986,1991,1996,2001,2006,2011},
y grid style={white},
ylabel={No Time

ROC\_AUC},
ymajorgrids,
ymin=-0.04764, ymax=1.00044,
ytick style={color=white!33.3333333333333!black},
ytick={0,0.05,0.1,0.15,0.2,0.25,0.3,0.35,0.4,0.45,0.5,0.55,0.6,0.65,0.7,0.75,0.8,0.85,0.9,0.95,1},
yticklabels={0.0,0.05,0.1,0.15,0.2,0.25,0.3,0.35,0.4,0.45,0.5,0.55,0.6,0.65,0.7,0.75,0.8,0.85,0.9,0.95,1.0}
]
\addplot [red, dotted]
table {%
0 0.7892
1 0.7996
2 0.7891
3 0.7895
4 0.7951
5 0.805
6 0.7973
7 0.7965
8 0.7668
9 0.7689
10 0.7729
11 0.7749
};
\addplot [red]
table {%
0 0.7642
1 0.7563
2 0.7516
3 0.7471
4 0.7727
5 0.7908
6 0.7912
7 0.7873
8 0.8126
9 0.7987
10 0.9232
11 0
};
\addplot [very thick, blue, dotted]
table {%
0 0.9347
1 0.9339
2 0.9306
3 0.9303
4 0.9253
5 0.9306
6 0.9232
7 0.9217
8 0.9127
9 0.904
10 0.908
11 0.9052
};
\addplot [very thick, blue]
table {%
0 0.9272
1 0.9427
2 0.9431
3 0.9433
4 0.9479
5 0.9498
6 0.9486
7 0.9528
8 0.9425
9 0.9518
10 0.9507
11 0
};
\addplot [thick, black, dotted]
table {%
0 0.8527
1 0.8576
2 0.8571
3 0.8599
4 0.8505
5 0.8546
6 0.8551
7 0.8585
8 0.8194
9 0.824
10 0.8171
11 0.816
};
\addplot [thick, black]
table {%
0 0.845
1 0.8625
2 0.8669
3 0.8724
4 0.8718
5 0.8777
6 0.8707
7 0.8819
8 0.8572
9 0.851
10 0.7391
11 0
};
\draw ({$(current bounding box.south west)!0.5!(current bounding box.south east)$}|-{$(current bounding box.south west)!0.98!(current bounding box.north west)$}) node[
  scale=0.6,
  anchor=north,
  text=black,
  rotate=0.0
]{pretrained};
\end{groupplot}

\end{tikzpicture}


==> link_prediction/tex/random.tex <==
% This file was created with tikzplotlib v0.9.12.
\begin{tikzpicture}

\begin{groupplot}[group style={group size=2 by 2}]
\nextgroupplot[
axis background/.style={fill=white!89.8039215686275!black},
axis line style={white},
tick align=outside,
tick pos=left,
title={Remove Acts
},
x grid style={white},
xmajorgrids,
xmin=-0.55, xmax=11.55,
xtick style={color=white!33.3333333333333!black},
xtick={0,1,2,3,4,5,6,7,8,9,10,11},
xtick={0,1,2,3,4,5,6,7,8,9,10,11},
xtick={0,1,2,3,4,5,6,7,8,9,10,11},
xtick={0,1,2,3,4,5,6,7,8,9,10,11},
xtick={0,1,2,3,4,5,6,7,8,9,10,11},
xtick={0,1,2,3,4,5,6,7,8,9,10,11},
xtick={0,1,2,3,4,5,6,7,8,9,10,11},
xticklabels={1956,1961,1966,1971,1976,1981,1986,1991,1996,2001,2006,2011},
xticklabels={1956,1961,1966,1971,1976,1981,1986,1991,1996,2001,2006,2011},
xticklabels={1956,1961,1966,1971,1976,1981,1986,1991,1996,2001,2006,2011},
xticklabels={1956,1961,1966,1971,1976,1981,1986,1991,1996,2001,2006,2011},
xticklabels={1956,1961,1966,1971,1976,1981,1986,1991,1996,2001,2006,2011},
xticklabels={1956,1961,1966,1971,1976,1981,1986,1991,1996,2001,2006,2011},
xticklabels={1956,1961,1966,1971,1976,1981,1986,1991,1996,2001,2006,2011},
y grid style={white},
ymajorgrids,
ymin=-0.047675, ymax=1.001175,
ytick style={color=white!33.3333333333333!black},
ytick={-0.2,0,0.2,0.4,0.6,0.8,1,1.2},
yticklabels={−0.2,0.0,0.2,0.4,0.6,0.8,1.0,1.2}
]
\addplot [red, dotted]
table {%
0 0.8493
1 0.7915
2 0.7776
3 0.7769
4 0.7753
5 0.7853
6 0.7823
7 0.7825
8 0.7823
9 0.7851
10 0.7862
11 0.782
};
\addplot [red]
table {%
0 0.7689
1 0.7704
2 0.764
3 0.7588
4 0.7527
5 0.7585
6 0.7855
7 0.7948
8 0.8762
9 0.8873
10 0.9004
11 0
};
\addplot [very thick, blue, dotted]
table {%
0 0.9336
1 0.8982
2 0.8938
3 0.8946
4 0.893
5 0.8937
6 0.8965
7 0.8922
8 0.8939
9 0.8958
10 0.8918
11 0.8919
};
\addplot [very thick, blue]
table {%
0 0.8921
1 0.8925
2 0.8981
3 0.8966
4 0.8918
5 0.8957
6 0.9005
7 0.9116
8 0.9363
9 0.9505
10 0.9535
11 0
};
\addplot [thick, black, dotted]
table {%
0 0.8048
1 0.7995
2 0.7933
3 0.7858
4 0.7748
5 0.7651
6 0.7634
7 0.762
8 0.7635
9 0.7656
10 0.7638
11 0.7611
};
\addplot [thick, black]
table {%
0 0.7476
1 0.7625
2 0.7719
3 0.7783
4 0.7811
5 0.7791
6 0.7798
7 0.7628
8 0.7499
9 0.7417
10 0.8007
11 0
};

\nextgroupplot[
axis background/.style={fill=white!89.8039215686275!black},
axis line style={white},
tick align=outside,
tick pos=left,
title={Keep Acts
},
x grid style={white},
xmajorgrids,
xmin=-0.55, xmax=11.55,
xtick style={color=white!33.3333333333333!black},
xtick={0,1,2,3,4,5,6,7,8,9,10,11},
xtick={0,1,2,3,4,5,6,7,8,9,10,11},
xtick={0,1,2,3,4,5,6,7,8,9,10,11},
xtick={0,1,2,3,4,5,6,7,8,9,10,11},
xtick={0,1,2,3,4,5,6,7,8,9,10,11},
xtick={0,1,2,3,4,5,6,7,8,9,10,11},
xtick={0,1,2,3,4,5,6,7,8,9,10,11},
xticklabel style={rotate=90.0},
xticklabels={1956,1961,1966,1971,1976,1981,1986,1991,1996,2001,2006,2011},
xticklabels={1956,1961,1966,1971,1976,1981,1986,1991,1996,2001,2006,2011},
xticklabels={1956,1961,1966,1971,1976,1981,1986,1991,1996,2001,2006,2011},
xticklabels={1956,1961,1966,1971,1976,1981,1986,1991,1996,2001,2006,2011},
xticklabels={1956,1961,1966,1971,1976,1981,1986,1991,1996,2001,2006,2011},
xticklabels={1956,1961,1966,1971,1976,1981,1986,1991,1996,2001,2006,2011},
xticklabels={1956,1961,1966,1971,1976,1981,1986,1991,1996,2001,2006,2011},
y grid style={white},
ylabel={Yes Time

ROC\_AUC},
ymajorgrids,
ymin=-0.04653, ymax=1,
ytick style={color=white!33.3333333333333!black},
ytick={0,0.05,0.1,0.15,0.2,0.25,0.3,0.35,0.4,0.45,0.5,0.55,0.6,0.65,0.7,0.75,0.8,0.85,0.9,0.95,1},
yticklabels={0.0,0.05,0.1,0.15,0.2,0.25,0.3,0.35,0.4,0.45,0.5,0.55,0.6,0.65,0.7,0.75,0.8,0.85,0.9,0.95,1.0}
]
\addplot [red, dotted]
table {%
0 0.7145
1 0.7007
2 0.697
3 0.6988
4 0.7017
5 0.7048
6 0.712
7 0.7065
8 0.711
9 0.717
10 0.7158
11 0.7135
};
\addplot [red]
table {%
0 0.7034
1 0.6952
2 0.6831
3 0.6905
4 0.6873
5 0.6788
6 0.6806
7 0.6789
8 0.7553
9 0.7298
10 0.8749
11 0
};
\addplot [very thick, blue, dotted]
table {%
0 0.9285
1 0.9101
2 0.8891
3 0.8731
4 0.8615
5 0.8467
6 0.8447
7 0.8475
8 0.8395
9 0.8388
10 0.8357
11 0.8366
};
\addplot [very thick, blue]
table {%
0 0.8449
1 0.8665
2 0.8804
3 0.8871
4 0.8936
5 0.9025
6 0.9154
7 0.9269
8 0.919
9 0.9261
10 0.9306
11 0
};
\addplot [thick, black, dotted]
table {%
0 0.8529
1 0.8372
2 0.8248
3 0.8111
4 0.8009
5 0.7818
6 0.7593
7 0.7246
8 0.6848
9 0.6836
10 0.6846
11 0.6829
};
\addplot [thick, black]
table {%
0 0.7607
1 0.8001
2 0.817
3 0.8224
4 0.8313
5 0.8353
6 0.847
7 0.8645
8 0.8372
9 0.8418
10 0.7282
11 0
};

\nextgroupplot[
axis background/.style={fill=white!89.8039215686275!black},
axis line style={white},
tick align=outside,
tick pos=left,
x grid style={white},
xmajorgrids,
xmin=-0.55, xmax=11.55,
xtick style={color=white!33.3333333333333!black},
xtick={0,1,2,3,4,5,6,7,8,9,10,11},
xtick={0,1,2,3,4,5,6,7,8,9,10,11},
xtick={0,1,2,3,4,5,6,7,8,9,10,11},
xtick={0,1,2,3,4,5,6,7,8,9,10,11},
xtick={0,1,2,3,4,5,6,7,8,9,10,11},
xtick={0,1,2,3,4,5,6,7,8,9,10,11},
xtick={0,1,2,3,4,5,6,7,8,9,10,11},
xticklabel style={rotate=90.0},
xticklabels={1956,1961,1966,1971,1976,1981,1986,1991,1996,2001,2006,2011},
xticklabels={1956,1961,1966,1971,1976,1981,1986,1991,1996,2001,2006,2011},
xticklabels={1956,1961,1966,1971,1976,1981,1986,1991,1996,2001,2006,2011},
xticklabels={1956,1961,1966,1971,1976,1981,1986,1991,1996,2001,2006,2011},
xticklabels={1956,1961,1966,1971,1976,1981,1986,1991,1996,2001,2006,2011},
xticklabels={1956,1961,1966,1971,1976,1981,1986,1991,1996,2001,2006,2011},
xticklabels={1956,1961,1966,1971,1976,1981,1986,1991,1996,2001,2006,2011},
y grid style={white},
ymajorgrids,
ymin=-0.04682, ymax=0.98322,
ytick style={color=white!33.3333333333333!black},
ytick={-0.2,0,0.2,0.4,0.6,0.8,1},
yticklabels={−0.2,0.0,0.2,0.4,0.6,0.8,1.0}
]
\addplot [red, dotted]
table {%
0 0.8546
1 0.8089
2 0.8016
3 0.8039
4 0.8051
5 0.8121
6 0.8178
7 0.8193
8 0.8221
9 0.8232
10 0.8221
11 0.8228
};
\addplot [red]
table {%
0 0.8077
1 0.8052
2 0.795
3 0.786
4 0.7869
5 0.7929
6 0.8231
7 0.8404
8 0.9121
9 0.9219
10 0
11 0
};
\addplot [very thick, blue, dotted]
table {%
0 0.9362
1 0.9155
2 0.9045
3 0.8992
4 0.8919
5 0.8845
6 0.8746
7 0.8754
8 0.8762
9 0.8782
10 0.8773
11 0.8772
};
\addplot [very thick, blue]
table {%
0 0.8855
1 0.8992
2 0.9077
3 0.9124
4 0.919
5 0.9254
6 0.9294
7 0.9262
8 0.9186
9 0.9364
10 0
11 0
};
\addplot [thick, black, dotted]
table {%
0 0.8113
1 0.8167
2 0.8178
3 0.8124
4 0.8025
5 0.788
6 0.7749
7 0.7744
8 0.7777
9 0.7758
10 0.7747
11 0.7747
};
\addplot [thick, black]
table {%
0 0.7741
1 0.7953
2 0.8097
3 0.8169
4 0.8176
5 0.817
6 0.8066
7 0.7986
8 0.7496
9 0.7435
10 0
11 0
};
\end{groupplot}

\begin{groupplot}[group style={group size=2 by 2}]
\nextgroupplot[
axis background/.style={fill=white!89.8039215686275!black},
axis line style={white},
tick align=outside,
tick pos=left,
x grid style={white},
xmajorgrids,
xmin=-0.55, xmax=11.55,
xtick style={color=white!33.3333333333333!black},
xtick={0,1,2,3,4,5,6,7,8,9,10,11},
xtick={0,1,2,3,4,5,6,7,8,9,10,11},
xtick={0,1,2,3,4,5,6,7,8,9,10,11},
xtick={0,1,2,3,4,5,6,7,8,9,10,11},
xtick={0,1,2,3,4,5,6,7,8,9,10,11},
xtick={0,1,2,3,4,5,6,7,8,9,10,11},
xtick={0,1,2,3,4,5,6,7,8,9,10,11},
xticklabel style={rotate=90.0},
xticklabels={1956,1961,1966,1971,1976,1981,1986,1991,1996,2001,2006,2011},
xticklabels={1956,1961,1966,1971,1976,1981,1986,1991,1996,2001,2006,2011},
xticklabels={1956,1961,1966,1971,1976,1981,1986,1991,1996,2001,2006,2011},
xticklabels={1956,1961,1966,1971,1976,1981,1986,1991,1996,2001,2006,2011},
xticklabels={1956,1961,1966,1971,1976,1981,1986,1991,1996,2001,2006,2011},
xticklabels={1956,1961,1966,1971,1976,1981,1986,1991,1996,2001,2006,2011},
xticklabels={1956,1961,1966,1971,1976,1981,1986,1991,1996,2001,2006,2011},
y grid style={white},
ylabel={No Time

ROC\_AUC},
ymajorgrids,
ymin=-0.04688, ymax=1,
ytick style={color=white!33.3333333333333!black},
ytick={0,0.05,0.1,0.15,0.2,0.25,0.3,0.35,0.4,0.45,0.5,0.55,0.6,0.65,0.7,0.75,0.8,0.85,0.9,0.95,1},
yticklabels={0.0,0.05,0.1,0.15,0.2,0.25,0.3,0.35,0.4,0.45,0.5,0.55,0.6,0.65,0.7,0.75,0.8,0.85,0.9,0.95,1.0}
]
\addplot [red, dotted]
table {%
0 0.7133
1 0.7073
2 0.7036
3 0.7011
4 0.7014
5 0.704
6 0.7059
7 0.7141
8 0.7154
9 0.7198
10 0.7186
11 0.7184
};
\addplot [red]
table {%
0 0.7011
1 0.6957
2 0.6903
3 0.6854
4 0.6855
5 0.6717
6 0.6908
7 0.6805
8 0.7614
9 0.7547
10 0.8541
11 0
};
\addplot [very thick, blue, dotted]
table {%
0 0.9208
1 0.9137
2 0.8998
3 0.8916
4 0.8797
5 0.861
6 0.8399
7 0.8364
8 0.8376
9 0.8387
10 0.8349
11 0.8383
};
\addplot [very thick, blue]
table {%
0 0.8632
1 0.8994
2 0.9154
3 0.9193
4 0.9215
5 0.9268
6 0.9351
7 0.9376
8 0.9106
9 0.9119
10 0
11 0
};
\addplot [thick, black, dotted]
table {%
0 0.8564
1 0.8491
2 0.8387
3 0.8266
4 0.8073
5 0.7847
6 0.7544
7 0.7233
8 0.6915
9 0.6912
10 0.69
11 0.6896
};
\addplot [thick, black]
table {%
0 0.7681
1 0.8205
2 0.8362
3 0.8486
4 0.8544
5 0.8601
6 0.8641
7 0.8738
8 0.834
9 0.8443
10 0
11 0
};
\draw ({$(current bounding box.south west)!0.5!(current bounding box.south east)$}|-{$(current bounding box.south west)!0.98!(current bounding box.north west)$}) node[
  scale=0.6,
  anchor=north,
  text=black,
  rotate=0.0
]{random};
\end{groupplot}

\end{tikzpicture}


==> link_prediction/tex/vanilla.tex <==
% This file was created with tikzplotlib v0.9.12.
\begin{tikzpicture}

\begin{groupplot}[group style={group size=2 by 2}]
\nextgroupplot[
axis background/.style={fill=white!89.8039215686275!black},
axis line style={white},
tick align=outside,
tick pos=left,
title={Remove Acts
},
x grid style={white},
xmajorgrids,
xmin=-0.55, xmax=11.55,
xtick style={color=white!33.3333333333333!black},
xtick={0,1,2,3,4,5,6,7,8,9,10,11},
xtick={0,1,2,3,4,5,6,7,8,9,10,11},
xtick={0,1,2,3,4,5,6,7,8,9,10,11},
xtick={0,1,2,3,4,5,6,7,8,9,10,11},
xtick={0,1,2,3,4,5,6,7,8,9,10,11},
xtick={0,1,2,3,4,5,6,7,8,9,10,11},
xtick={0,1,2,3,4,5,6,7,8,9,10,11},
xticklabels={1956,1961,1966,1971,1976,1981,1986,1991,1996,2001,2006,2011},
xticklabels={1956,1961,1966,1971,1976,1981,1986,1991,1996,2001,2006,2011},
xticklabels={1956,1961,1966,1971,1976,1981,1986,1991,1996,2001,2006,2011},
xticklabels={1956,1961,1966,1971,1976,1981,1986,1991,1996,2001,2006,2011},
xticklabels={1956,1961,1966,1971,1976,1981,1986,1991,1996,2001,2006,2011},
xticklabels={1956,1961,1966,1971,1976,1981,1986,1991,1996,2001,2006,2011},
xticklabels={1956,1961,1966,1971,1976,1981,1986,1991,1996,2001,2006,2011},
y grid style={white},
ymajorgrids,
ymin=-0.048275, ymax=1.013775,
ytick style={color=white!33.3333333333333!black},
ytick={-0.2,0,0.2,0.4,0.6,0.8,1,1.2},
yticklabels={−0.2,0.0,0.2,0.4,0.6,0.8,1.0,1.2}
]
\addplot [red, dotted]
table {%
0 0.8885
1 0.8506
2 0.8295
3 0.8192
4 0.8211
5 0.8168
6 0.8124
7 0.8098
8 0.8109
9 0.8078
10 0.8103
11 0.814
};
\addplot [red]
table {%
0 0.8042
1 0.7997
2 0.7957
3 0.8005
4 0.8059
5 0.8163
6 0.83
7 0.8441
8 0.8966
9 0.9253
10 0
11 0
};
\addplot [very thick, blue, dotted]
table {%
0 0.9464
1 0.9426
2 0.9124
3 0.9095
4 0.9203
5 0.9172
6 0.9147
7 0.9123
8 0.914
9 0.9246
10 0.9245
11 0.9341
};
\addplot [very thick, blue]
table {%
0 0.913
1 0.9136
2 0.9041
3 0.9245
4 0.9285
5 0.9316
6 0.9396
7 0.9466
8 0.9622
9 0.9655
10 0
11 0
};
\addplot [thick, black, dotted]
table {%
0 0.7995
1 0.8257
2 0.8068
3 0.8176
4 0.8212
5 0.8247
6 0.8291
7 0.8349
8 0.838
9 0.8399
10 0.8439
11 0.8455
};
\addplot [thick, black]
table {%
0 0.8323
1 0.8249
2 0.8322
3 0.8345
4 0.8376
5 0.8471
6 0.8398
7 0.8398
8 0.805
9 0.7867
10 0
11 0
};

\nextgroupplot[
axis background/.style={fill=white!89.8039215686275!black},
axis line style={white},
tick align=outside,
tick pos=left,
title={Keep Acts
},
x grid style={white},
xmajorgrids,
xmin=-0.55, xmax=11.55,
xtick style={color=white!33.3333333333333!black},
xtick={0,1,2,3,4,5,6,7,8,9,10,11},
xtick={0,1,2,3,4,5,6,7,8,9,10,11},
xtick={0,1,2,3,4,5,6,7,8,9,10,11},
xtick={0,1,2,3,4,5,6,7,8,9,10,11},
xtick={0,1,2,3,4,5,6,7,8,9,10,11},
xtick={0,1,2,3,4,5,6,7,8,9,10,11},
xtick={0,1,2,3,4,5,6,7,8,9,10,11},
xticklabel style={rotate=90.0},
xticklabels={1956,1961,1966,1971,1976,1981,1986,1991,1996,2001,2006,2011},
xticklabels={1956,1961,1966,1971,1976,1981,1986,1991,1996,2001,2006,2011},
xticklabels={1956,1961,1966,1971,1976,1981,1986,1991,1996,2001,2006,2011},
xticklabels={1956,1961,1966,1971,1976,1981,1986,1991,1996,2001,2006,2011},
xticklabels={1956,1961,1966,1971,1976,1981,1986,1991,1996,2001,2006,2011},
xticklabels={1956,1961,1966,1971,1976,1981,1986,1991,1996,2001,2006,2011},
xticklabels={1956,1961,1966,1971,1976,1981,1986,1991,1996,2001,2006,2011},
y grid style={white},
ylabel={Yes Time

ROC\_AUC},
ymajorgrids,
ymin=-0.047925, ymax=1.006425,
ytick style={color=white!33.3333333333333!black},
ytick={0,0.05,0.1,0.15,0.2,0.25,0.3,0.35,0.4,0.45,0.5,0.55,0.6,0.65,0.7,0.75,0.8,0.85,0.9,0.95,1},
yticklabels={0.0,0.05,0.1,0.15,0.2,0.25,0.3,0.35,0.4,0.45,0.5,0.55,0.6,0.65,0.7,0.75,0.8,0.85,0.9,0.95,1.0}
]
\addplot [red, dotted]
table {%
0 0.7898
1 0.8001
2 0.7879
3 0.7909
4 0.7922
5 0.7926
6 0.7962
7 0.7869
8 0.7629
9 0.7607
10 0.77
11 0.7708
};
\addplot [red]
table {%
0 0.7566
1 0.7574
2 0.7444
3 0.757
4 0.7775
5 0.7969
6 0.7961
7 0.8021
8 0.802
9 0.8138
10 0
11 0
};
\addplot [very thick, blue, dotted]
table {%
0 0.9482
1 0.9417
2 0.9231
3 0.9147
4 0.9207
5 0.9163
6 0.9173
7 0.9181
8 0.879
9 0.8956
10 0.8898
11 0.8828
};
\addplot [very thick, blue]
table {%
0 0.9113
1 0.9384
2 0.9427
3 0.9447
4 0.9476
5 0.9462
6 0.9505
7 0.9585
8 0.9384
9 0.9437
10 0
11 0
};
\addplot [thick, black, dotted]
table {%
0 0.8609
1 0.865
2 0.8527
3 0.8509
4 0.8519
5 0.8494
6 0.8527
7 0.8581
8 0.814
9 0.8229
10 0.8266
11 0.8253
};
\addplot [thick, black]
table {%
0 0.8422
1 0.8631
2 0.8627
3 0.8674
4 0.8782
5 0.8761
6 0.8825
7 0.8913
8 0.8724
9 0.8694
10 0
11 0
};

\nextgroupplot[
axis background/.style={fill=white!89.8039215686275!black},
axis line style={white},
tick align=outside,
tick pos=left,
x grid style={white},
xmajorgrids,
xmin=-0.55, xmax=11.55,
xtick style={color=white!33.3333333333333!black},
xtick={0,1,2,3,4,5,6,7,8,9,10,11},
xtick={0,1,2,3,4,5,6,7,8,9,10,11},
xtick={0,1,2,3,4,5,6,7,8,9,10,11},
xtick={0,1,2,3,4,5,6,7,8,9,10,11},
xtick={0,1,2,3,4,5,6,7,8,9,10,11},
xtick={0,1,2,3,4,5,6,7,8,9,10,11},
xtick={0,1,2,3,4,5,6,7,8,9,10,11},
xticklabel style={rotate=90.0},
xticklabels={1956,1961,1966,1971,1976,1981,1986,1991,1996,2001,2006,2011},
xticklabels={1956,1961,1966,1971,1976,1981,1986,1991,1996,2001,2006,2011},
xticklabels={1956,1961,1966,1971,1976,1981,1986,1991,1996,2001,2006,2011},
xticklabels={1956,1961,1966,1971,1976,1981,1986,1991,1996,2001,2006,2011},
xticklabels={1956,1961,1966,1971,1976,1981,1986,1991,1996,2001,2006,2011},
xticklabels={1956,1961,1966,1971,1976,1981,1986,1991,1996,2001,2006,2011},
xticklabels={1956,1961,1966,1971,1976,1981,1986,1991,1996,2001,2006,2011},
y grid style={white},
ymajorgrids,
ymin=-0.048, ymax=1.008,
ytick style={color=white!33.3333333333333!black},
ytick={-0.2,0,0.2,0.4,0.6,0.8,1,1.2},
yticklabels={−0.2,0.0,0.2,0.4,0.6,0.8,1.0,1.2}
]
\addplot [red, dotted]
table {%
0 0.9021
1 0.8812
2 0.8673
3 0.8647
4 0.8707
5 0.8776
6 0.8748
7 0.8676
8 0.866
9 0.8635
10 0.8627
11 0.861
};
\addplot [red]
table {%
0 0.8667
1 0.8611
2 0.861
3 0.8577
4 0.8647
5 0.8827
6 0.8981
7 0.9082
8 0.9538
9 0.9549
10 0
11 0
};
\addplot [very thick, blue, dotted]
table {%
0 0.947
1 0.9455
2 0.9394
3 0.9386
4 0.9382
5 0.9378
6 0.9339
7 0.9313
8 0.9256
9 0.9212
10 0.9307
11 0.9143
};
\addplot [very thick, blue]
table {%
0 0.9373
1 0.9409
2 0.9397
3 0.9426
4 0.9461
5 0.9477
6 0.9513
7 0.9557
8 0.96
9 0.9549
10 0
11 0
};
\addplot [thick, black, dotted]
table {%
0 0.8379
1 0.851
2 0.8587
3 0.856
4 0.8602
5 0.8579
6 0.8584
7 0.8471
8 0.8333
9 0.8313
10 0.8296
11 0.8277
};
\addplot [thick, black]
table {%
0 0.8507
1 0.8621
2 0.8644
3 0.8643
4 0.8661
5 0.8626
6 0.8605
7 0.8492
8 0.834
9 0.8203
10 0
11 0
};
\end{groupplot}

\begin{groupplot}[group style={group size=2 by 2}]
\nextgroupplot[
axis background/.style={fill=white!89.8039215686275!black},
axis line style={white},
tick align=outside,
tick pos=left,
x grid style={white},
xmajorgrids,
xmin=-0.55, xmax=11.55,
xtick style={color=white!33.3333333333333!black},
xtick={0,1,2,3,4,5,6,7,8,9,10,11},
xtick={0,1,2,3,4,5,6,7,8,9,10,11},
xtick={0,1,2,3,4,5,6,7,8,9,10,11},
xtick={0,1,2,3,4,5,6,7,8,9,10,11},
xtick={0,1,2,3,4,5,6,7,8,9,10,11},
xtick={0,1,2,3,4,5,6,7,8,9,10,11},
xtick={0,1,2,3,4,5,6,7,8,9,10,11},
xticklabel style={rotate=90.0},
xticklabels={1956,1961,1966,1971,1976,1981,1986,1991,1996,2001,2006,2011},
xticklabels={1956,1961,1966,1971,1976,1981,1986,1991,1996,2001,2006,2011},
xticklabels={1956,1961,1966,1971,1976,1981,1986,1991,1996,2001,2006,2011},
xticklabels={1956,1961,1966,1971,1976,1981,1986,1991,1996,2001,2006,2011},
xticklabels={1956,1961,1966,1971,1976,1981,1986,1991,1996,2001,2006,2011},
xticklabels={1956,1961,1966,1971,1976,1981,1986,1991,1996,2001,2006,2011},
xticklabels={1956,1961,1966,1971,1976,1981,1986,1991,1996,2001,2006,2011},
y grid style={white},
ylabel={No Time

ROC\_AUC},
ymajorgrids,
ymin=-0.04792, ymax=1.00632,
ytick style={color=white!33.3333333333333!black},
ytick={0,0.05,0.1,0.15,0.2,0.25,0.3,0.35,0.4,0.45,0.5,0.55,0.6,0.65,0.7,0.75,0.8,0.85,0.9,0.95,1},
yticklabels={0.0,0.05,0.1,0.15,0.2,0.25,0.3,0.35,0.4,0.45,0.5,0.55,0.6,0.65,0.7,0.75,0.8,0.85,0.9,0.95,1.0}
]
\addplot [red, dotted]
table {%
0 0.8055
1 0.8146
2 0.7993
3 0.805
4 0.8131
5 0.8099
6 0.8151
7 0.8051
8 0.7859
9 0.7846
10 0.7846
11 0.7855
};
\addplot [red]
table {%
0 0.778
1 0.7813
2 0.7658
3 0.7708
4 0.7981
5 0.8202
6 0.8254
7 0.8075
8 0.8175
9 0.796
10 0
11 0
};
\addplot [very thick, blue, dotted]
table {%
0 0.9428
1 0.9445
2 0.9375
3 0.9321
4 0.9307
5 0.9309
6 0.9249
7 0.9258
8 0.9
9 0.8954
10 0.8797
11 0.8875
};
\addplot [very thick, blue]
table {%
0 0.9247
1 0.944
2 0.9474
3 0.9498
4 0.9482
5 0.9548
6 0.9565
7 0.9584
8 0.9404
9 0.9477
10 0
11 0
};
\addplot [thick, black, dotted]
table {%
0 0.8726
1 0.878
2 0.8693
3 0.8718
4 0.8661
5 0.8618
6 0.8621
7 0.8613
8 0.8225
9 0.8256
10 0.8159
11 0.8184
};
\addplot [thick, black]
table {%
0 0.8514
1 0.8721
2 0.8751
3 0.8854
4 0.8872
5 0.8877
6 0.8886
7 0.8981
8 0.8729
9 0.8725
10 0
11 0
};
\draw ({$(current bounding box.south west)!0.5!(current bounding box.south east)$}|-{$(current bounding box.south west)!0.98!(current bounding box.north west)$}) node[
  scale=0.6,
  anchor=north,
  text=black,
  rotate=0.0
]{vanilla};
\end{groupplot}

\end{tikzpicture}

